Combining SMT and NMT Back-Translated Data for Efficient NMT

Neural Machine Translation (NMT) models achieve their best performance when large sets of parallel data are used for training. Consequently, techniques for augmenting the training set have become popular recently. One of these methods is back-translation (Sennrich et al., 2016), which consists on generating synthetic sentences by translating a set of monolingual, target-language sentences using a Machine Translation (MT) model. Generally, NMT models are used for back-translation. In this work, we analyze the performance of models when the training data is extended with synthetic data using different MT approaches. In particular we investigate back-translated data generated not only by NMT but also by Statistical Machine Translation (SMT) models and combinations of both. The results reveal that the models achieve the best performances when the training set is augmented with back-translated data created by merging different MT approaches.

==> old_tables.tex <==

\begin{table*}[!htbp]
\centering
\begin{tabular}{|p{0.25cm}|p{2cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{3cm}|}
\hline
&	&	 1M \textit{base}.  	&	-  	&	-  	&	-	\\
\hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering 1M lines}}	
& BLEU$\uparrow$	&	0.234	&	-	&	-	&	-	\\
%& NIST$\uparrow$	&	-	&	-	&	-	&	-	\\
& TER$\downarrow$ 	&	0.5723	&	-	&	-	&	-	\\
& METEOR$\uparrow$	&	0.2809	&	-	&	-	&	-	\\
%& {\small CHR}F3$\uparrow$	&	-	&	-	&	-	&	-	\\
&{\small CHR}F1$\uparrow$	&	50.6643	&	-	&	-	&	-	\\
\hline									
&	&	 1M \textit{base} +1M \textit{auth}  	&	 1M \textit{base} +1M \textit{NMTsynth} 	&	1M \textit{base} + 1M \textit{SMTsynth}	&	1M \textit{base} + 1M \textit{hybrNMTSMT}			\\
\hline									
\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering 2M lines}}	
& BLEU$\uparrow$	&	0.2487	&	0.2532	&	0.2438	&	0.2521	\\
%& NIST$\uparrow$	&	7.1388	&	7.1889	&	7.0872	&	7.1827	\\
& TER$\downarrow$ 	&	0.5581	&	0.5566	&	0.5605	&	0.5587	\\
& METEOR$\uparrow$	&	0.2916	&	0.2933	&	0.2893	&	0.2929	\\
%& {\small CHR}F3$\uparrow$	&	50.1831	&	50.6275	&	49.9941	&	50.6926	\\
&{\small CHR}F1$\uparrow$	&	52.0346	&	52.2511	&	51.887	&	52.3621	\\
\hline									
&	&	 1M \textit{base} +2M \textit{auth}.  	&	 1M \textit{base} + 2M \textit{NMTsynth}	&	 1M \textit{base} + 2M \textit{SMTsynth}		&	1M \textit{base} + 2M \textit{hybrNMTSMT} \\
\hline									
\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering 3M lines}}	
& BLEU$\uparrow$	&	0.2569	&	0.2544	&	0.2458	&	0.2562	\\
%& NIST$\uparrow$	&	7.2585	&	7.2203	&	7.1263	&	7.2812	\\
& TER$\downarrow$ 	&	0.5499	&	0.5562	&	0.557	&	0.5525	\\
& METEOR$\uparrow$	&	0.2970	&	0.2947	&	0.2902	&	0.2973	\\
%& {\small CHR}F3$\uparrow$	&	50.9854	&	50.9214	&	50.1128	&	51.3724	\\
& {\small CHR}F1$\uparrow$	&	52.7697	&	52.5008	&	52.0854	&	52.8867	\\
\hline									
&	&	1M \textit{base} +3M \textit{auth}	&	 1M \textit{base} + 3M \textit{NMTsynth}	&	 1M \textit{base} + 3M \textit{SMTsynth}	&	1M \textit{base} +3M  \textit{hybrNMTSMT}	\\
\hline									
\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering 4M lines}}	
& BLEU$\uparrow$	&	0.2597	&	0.2601	&	0.2465	&	0.2583	\\
%& NIST$\uparrow$	&	7.313	&	7.2876	&	7.1447	&	7.2769	\\
& TER$\downarrow$ 	&	0.5454	&	0.5533	&	0.5558	&	0.5517	\\
& METEOR$\uparrow$	&	0.2991	&	0.2971	&	0.2926	&	0.2974	\\
%& {\small CHR}F3$\uparrow$	&	51.3745	&	51.2344	&	50.3382	&	51.3283	\\
&{\small CHR}F1$\uparrow$	&	53.1585	&	52.8667	&	52.2441	&	52.8375	\\
\hline							
\end{tabular}
\caption{Performance of models built with different sizes of authentic and synthetic data.  \label{table:results}}
\end{table*}














\begin{table*}[!htbp]
\centering
\begin{tabular}{|p{1.5cm}|p{0.25cm}|p{2.2cm}|p{2.2cm}|p{2.2cm}|p{2.2cm}||p{0.2cm}|p{2.2cm}|}
\hline
&	&	 1M \textit{base} +1M \textit{auth}  	&	1M \textit{base} + 1M \textit{SMTsynth}	&	 1M \textit{base} +1M \textit{NMTsynth} 	&	1M \textit{base} + 1M \textit{hybrNMTSMT}	&&	1M \textit{base} + 2M \textit{fullhybrNMTSMT}	\\
\hline											
&\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering 2M lines}}	&&&&& \multirow{4}{*}{\rotatebox[origin=c]{90}{\centering 3M lines}} &\\
BLEU$\uparrow$	&&	24.87	&	24.38	&	25.32	&	25.21	&&	25.34	\\
%& NIST$\uparrow$	&&	7.1388	&	7.0872	&	7.1889	&	7.1827	&	7.2151	\\
 TER$\downarrow$ 	&&	55.81	&	56.05	&	55.66	&	55.87	&&	55.79	\\
 METEOR$\uparrow$	&&	29.16	&	28.93	&	29.33	&	29.29	&&	29.47	\\
%& {\small CHR}F3$\uparrow$	&&	50.1831	&	49.9941	&	50.6275	&	50.6926	&	50.9642	\\
{\small CHR}F1$\uparrow$	&&	52.03	&	51.89	&	52.25	&	52.36	&&	52.47	\\
\hline							
\end{tabular}
\caption{Performance of models built with different sizes of authentic and synthetic data.  \label{table:results}}
\end{table*}



